Properties of minimally doubled fermions

Most quark actions in lattice QCD encounter difficulties with chiral symmetry and its spontaneous breakdown. Minimally doubled fermions (MDF) are a category of strictly local chiral lattice fermions, whose continuum limit reproduces two degenerate quark flavours. The two poles of their Dirac operator are aligned such that symmetries under charge conjugation or reflection of one particular direction are explictly broken at finite lattice spacing. Properties of MDF are scrutinised with regard to broken symmetry and meson spectrum to discern their suitability for numerical studies of QCD. Interactions induce anisotropic operator mixing for MDF. Hence, restoration of broken symmetries in the continuum limit requires three counterterms, one of which is power-law divergent. Counterterms and operator mixing are studied perturbatively for two variants of MDF. Two independent non-perturbative procedures for removal of the power-law divergence are developed by means of a numerical study of hadronic observables for one variant of MDF in quenched approximation. Though three out of four pseudoscalar mesons are affected by lattice artefacts, the spectrum's continuum limit is consistent with two-flavour QCD. Thus, suitability of MDF for numerical studies of QCD in the quenched approximation is demonstrated.

==> acknowledgements.tex <==

{\centering\textbf{In memoriam of my grandparents Marianne and Karl Schenkel}\par}
\vskip1em

\noindent
First and foremost, I dedicate my thesis to the memory of my late grandmother -- visiting her in her last days instead of concentrating on my thesis is still one of the best choices of my life -- and my grandfather, who started a doctoral thesis twice -- and twice it was annihilated as his home was destroyed by bombs during the war. He didn't restart again. 
\vskip1em

\noindent
I have to acknowledge my gratitude to my primary supervisor Hartmut Wittig, who inspired me to take up lattice QCD for my PhD. His support was vital during these years. He also introduced me to Sinya Aoki, my second supervisor during my time in Tsukuba, to whom I am also greatly indebted for his unwavering support. I'd like to thank Stefano Capitani and Georg von Hippel for invaluable advice and for teaching me large parts of what I know about the lattice. I am very thankful to Michael Creutz for again bringing up minimally doubled fermions just at the right time for me to jump on the topic. My teachers taught me a lot that I -- and maybe they -- have not expected. 
I also have to thank Christian Seiwerth at the Institut f\"{u}r Kernphysik at Johannes Gutenberg-Universit\"{a}t Mainz for technical support. For financial support, my thanks go to DFG (SFB 1044), GSI, EMG, DAAD, MEXT and A4 collaboration. %\newline
\noindent
I owe a lot to Frank Maas, Sebastian Baunack and the A4 collaboration for having me -- a theoretician -- as a HIWI at different times and bringing out my interest in experimental physics anew. Furthermore, I'd like to express profound thanks to Martin Reuter and Frank Maas for their guidance when I needed it most. HGS-HIRe should not be forgotten as they disclosed new perspectives to me. 
I'd also like to articulate my appreciation towards Marc Wagner for putting me on the path of thermal field theory and to Nora Brambilla and Peter Petreczky for giving me the chance to work with them despite not having finished my PhD for a long year. For help with my Japanese that suffered during the last two years of my PhD, I'd like to thank Hana Saito and Marina Horonushi. 
\vskip1em

\noindent
Last but not least, I'd like to express heartfelt thanks to my parents for supporting me through 13 years of school and more than 11 years of university in every possible way. I thank my girlfriend Rebecca for being the silver lining on the horizon for each other.


==> fin_bibconventions.tex <==

\sectionc{Physical constants}{app: Physical constants}

\noindent
This section declares the unit conventions throughout this thesis. Natural units are applied throughout this thesis, i.e.
\begin{equation}
  c=1=\hbar.
\end{equation}
Therefore, physical quantities have the following length dimensions:
\begin{equation}
  [\text{length}] = [\text{time}] = [\text{energy}]^{-1} = [\text{mass}]^{-1}.
\end{equation}
For the purpose of conversion to other systems of units, the product of the quantum of action and the speed of light in vacuum as well as the speed of light in vacuum are given in SI units by
\begin{equation}
  \hbar c = 197.326968(17)\, \mathrm{MeV}\, \mathrm{fm},\quad
  c = 299792458\, \mathrm{m}\, \mathrm{s}^{-1}.
\end{equation}


\sectionc{Indices}{app: Indices}

\noindent
This section declares the index conventions throughout this thesis.

\subsubsection{Space-time indices}

\noindent
Space-time indices are labelled by Greek letters mostly from the middle of the Greek alphabet. If they are applied in Minkowski space-time $ \mathbb{M}^4 $, their range is $ \mu \in \{0,1,2,3\} $. If they are applied in Euclidean space-time $ \mathbb{R}^4 $, their range is $ \mu \in \{0,1,2,3\} $ as well. Space-time indices, which occur multiply are always considered to be summed over. Exceptions are explicitly highlighted. Fixed indices, which are never summed are marked by an underscore, e.g. $ \underline{\mu} $.

\subsubsection{Spinor indices}

\noindent
Spinor indices are labelled by Greek letters mostly from the beginning of the Greek alphabet. Their range is $ \alpha \in \{1,2,3,4\} $. Spinor indices which occur twice are always considered to be summed over according to Einstein's summation convention.

\subsubsection{Colour indices}

\noindent
Colour indices in the fundamental representation are labelled by Latin letters mostly from the start of the alphabet. The range of colour indices in the fundamental representation is $ a \in \{1,2,3\}$. Colour indices of the fields in the adjoint representation are labelled by bracketed Latin letters mostly from the start of the alphabet. The range of colour indices in the adjoint representation is $ (a) \in \{1,2,3,4,5,6,7,8\}$. Colour indices which occur twice in either the fundamental or adjoint representation are always considered to be summed over according to Einstein's summation convention. Exceptions are explicitly highlighted. Fixed indices, which are never summed are marked by an underscore, e.g. $ \underline{a} $.

\subsubsection{Flavour indices}

\noindent
Flavour indices in the fundamental representation are labelled by bracketed numbers. Their general range is $ f \in \{1,2,3,4,5,6\} $ and they are sorted in the order of ascending quark mass. The spinor's symbol $ \psi $ can be replaced by the one-letter label of the flavours, e.g. $ \psi^{(1)}\equiv u $, $ \psi^{(2)}\equiv d $, $ \ldots $ and the quark mass parameters can be labeled as $ m^{(1)}=m_u $, $ m^{(2)}=m_d $, $ \ldots $. Summation of flavour indices is always declared explicitly.

\subsubsection{Space-time coordinates}

\noindent
Space-time coordinates $ x $ of field variables $ \psi $ defined on a space-time continuum are represented as arguments of the fields, e.g. $ \psi(x) $. In the contrary, site labels $ n $ on discretised space-time $ n_\mu=x_\mu/a $, which are dimensionless numbers, are represented as site indices $ \psi_n $. Integration over space-time coordinates or summation over site labels are always declared explicitly.

\subsubsection{Momentum space coordinates}

\noindent
The vector space of four-momenta is referred to as momentum space throughout this thesis. Its coordinates $ k_\mu $ are always represented as arguments of the fields, $ \psi(k) $. Integration over momentum space coordinates is always declared explicitly.



\sectionc{\textit{ SU(N) }-Matrices}{app: SU(N)-Matrices}
\noindent
This section declares the conventions concerning $ SU(N) $ matrices.

\subsubsection{\textit{ SU(2) } -- Pauli matrices}
The Pauli matrices $ \sigma^{\mu} $ are defined by
\begin{equation}
  \sigma^1=\left(\begin{array}{cc} 0 & 1 \\ 1 & 0 \end{array}\right), \quad
  \sigma^2=\left(\begin{array}{cc} 0 & -i \\ i & 0 \end{array}\right), \quad
  \sigma^3=\left(\begin{array}{cc} 1 & 0 \\ 0 & -1 \end{array}\right).
\end{equation}
The $ 2\times2 $-unit matrix is included as
\begin{equation}
  \sigma^0=\left(\begin{array}{cc} 1 & 0 \\ 0 & 1 \end{array}\right).
\end{equation}
As generators of the symmetry group $ SU(2) $, they are defined with an additional factor $ 1/2 $,
\begin{equation}
  \tau_j=\frac{1}{2}\sigma^j
\end{equation}
and satisfy
\begin{equation}
  \tau^i \tau^j=\frac{1}{2}\left(\delta^{ij} +i\epsilon^{ijk}\tau^k\right).
\end{equation}

\subsubsection{\textit{ SU(3) } -- Gell-Mann matrices}
The Gell-Mann matrices $ \lambda^{j} $ are defined by
\small
\begin{align}
  \lambda^1=&\left(\begin{array}{ccc} 0 & 1 & 0 \\ 1 & 0 & 0 \\ 0 & 0 & 0 \end{array}\right), &&
  \lambda^2=&\left(\begin{array}{ccc} 0 & -i & 0 \\ i & 0 & 0 \\ 0 & 0 & 0 \end{array}\right), &&
  \lambda^3=&\left(\begin{array}{ccc} 1 & 0 & 0 \\ 0 & -1 & 0 \\ 0 & 0 & 0 \end{array}\right), \nonumber \\
  \lambda^4=&\left(\begin{array}{ccc} 0 & 0 & 1 \\ 0 & 0 & 0 \\ 1 & 0 & 0 \end{array}\right), &&
  \lambda^5=&\left(\begin{array}{ccc} 0 & 0 & -i \\ 0 & 0 & 0 \\ i & 0 & 0 \end{array}\right), &&
  \lambda^6=&\left(\begin{array}{ccc} 0 & 0 & 0 \\ 0 & 0 & 1 \\ 0 & 1 & 0 \end{array}\right), \nonumber \\
  \lambda^7=&\left(\begin{array}{ccc} 0 & 0 & 0 \\ 0 & 0 & -i \\ 0 & i & 0 \end{array}\right), &&
  \lambda^8=&\frac{1}{\sqrt{3}}\left(\begin{array}{ccc} 1 & 0 & 0 \\ 0 & 1 & 0 \\ 0 & 0 & -2 \end{array}\right). &&
\end{align}\normalsize
As generators of the symmetry group $ SU(3) $, they are defined with an additional factor $ 1/2 $,
\begin{equation}
  T_j=\frac{1}{2}\lambda^j
\end{equation}
and satisfy
\begin{equation}
  T^i T^j=\frac{1}{2}\left(\frac{1}{3}\delta^{ij}\mathbf{1}+(d^{ijk}+i f^{ijk})T_k\right).
  \label{eq: product of SU(3) generators}
\end{equation}

\subsubsection{Casimir operators}
The Casimir operators of the group $ SU(N) $ are given by
\begin{align}
  C(R)=&\ \frac{1}{2}
   = \mathrm{Tr}(T_{\underline{a}}T_{\underline{a}}) 
   \label{eq: Casimir operator C_2} \\ 
  C_2(R) 1_{N\times N}
  =&\ \sum\limits_{a}T_{a}T_{a}
   = \frac{N^2-1}{2N} 1_{N\times N},\quad C_2(R)\equiv C_F 
   \label{eq: Casimir operator C_F} \\ 
  C_2 \equiv C_2(G) 
  =&\ C(G) =f^{\underline{a}cd}f^{\underline{a}cd} = N,
\end{align}
where $ R $ is the fundamental and $ G $ is the adjoint representation.

\sectionc{Minkowski and Euclidean space-time}{app: Minkowski and Euclidean space-time}
\noindent
This section declares the conventions concerning Minkowski and Euclidean space-time throughout this thesis. Quantities defined on a Minkowski or Euclidean space-time are always labelled with upper indices $ M $ or $ E $ if there is any possibility of an ambiguity. If ambiguities can be excluded, the labels are omitted.

\subsection{Coordinates and four-vectors}
This thesis mostly uses Euclidean space-time. Four-vectors defined on Euclidean space-time are connected with four-vectors on Minkowski space-time by a Wick rotation. The Wick rotation of the $ x_0 $ coordinate is defined as
\begin{equation}
  x_0^E \equiv i x_0^M.
\end{equation}
The Minkowski space-time coordinate $ x_0^M $ is identical to the usual physical time $ t $. Four-momenta $ p_\mu $, derivatives $ \partial_\mu $ as well as four-vector fields $ A_\mu(x) $ have their temporal components transformed by the Wick-rotation with the conjugate factor $ (-i) $,
\begin{align}
  p_0^E =&\ -i p_0^M, \\
  \partial_0^E =\frac{\partial}{\partial x^{0\,E}} =&\ \frac{1}{i}\frac{\partial}{\partial x^{0\,M}} = -i \partial_0^M, 
  \label{eq: Wick rotation of derivatives} \\
  A_0^E(x^E) =&\ -i A_0^M(x^M) \label{eq: Wick rotation of vector fields}.
\end{align}
Four-vectors are defined in Minkowski and Euclidean space-time by
\begin{align}
  x^{M\,\mu} =&\ (x_0^M,\mathbf{x}^M), \\
  x_\mu^M=g_{\mu\nu}x^{M\,\mu} =&\ (x_0^M,-\mathbf{x}^M), \\
  x_\mu^E = x^{E\,\mu } =&\ (x_0^E,\mathbf{x}^E)
\end{align}
and scalar products are
\begin{align}
  x^M \cdot y^M =&\ x_\mu^M y^{M\,\mu} = (x_0^M y_0^M) - (\mathbf{x}^M \cdot \mathbf{y}^M), \\
  x^E \cdot y^E =&\ x_\mu^E y_\mu^E = (x_0^E y_0^E) + (\mathbf{x}^E \cdot \mathbf{y}^E).
\end{align}
$ 3 $-dimensional vectors are in bold print (e.g. $ \mathbf{x} $). The scalar product of four-vectors and three-vectors are both abbreviated as dot products. The metric of Minkowski space-time is defined as
\begin{equation}
  g_{\mu\nu}=\mathrm{diag}\,(+1,-1,-1,-1).
\end{equation}
Due to the aforementioned transformation properties of derivatives in eq. (\ref{eq: Wick rotation of derivatives}) and vector fields in eq. (\ref{eq: Wick rotation of vector fields}), the field strength tensor $ F_{\mu\nu}(x) $ transforms as
\begin{equation}
  F^{E\,\mu\nu}(x^E) = F^{E}_{\mu\nu}(x^E) 
  = (-i)^{(\delta^{\mu0}+\delta^{\nu0})}\ F^{M}_{\mu\nu}(x^M) 
  = i^{(\delta^{\mu0}+\delta^{\nu0})}\ F^{M\,\mu\nu}(x^M).
\end{equation}
Thus, the product $ F^E_{\mu\nu}(x^E)F^E_{\mu\nu}(x^E)=F^M_{\mu\nu}(x^M)F^{M\,\mu\nu}(x^M) $ is not multiplied by any additional factors in the Wick rotation.

Spinor fields and adjoint spinor fields are treated as independent degrees of freedom in the Osterwalder-Schrader approach \cite{Osterwalder:1973kn, Osterwalder:1973dx} to a Euclidean field theory, but are otherwise left unchanged:
% \small
\begin{equation}
  \psi^E(x^E) = \psi^M(x^M), \quad \bar\psi^E(x^E) = \bar\psi^M(x^M).
\end{equation}\normalsize
While this is not of particular importance in the path integral approach, which already treats $ \psi $ and $ \bar\psi $ as independent field in Minkowski space-time, the OS approach causes a loss of hermiticity for the Dirac action, which can be avoided by Waldron's elaborate scheme for the Wick rotation including spinor rotations \cite{vanNieuwenhuizen:1996ip,vanNieuwenhuizen:1996tv,Waldron:1997re}. Throughout this thesis, the OS approach to Euclidean field theories is applied.

\subsection{Dirac matrices}\label{app: Dirac matrices}
Dirac matrices are defined as
% \small
\begin{align}
  \gamma^{M\,0}=&\ \left(\begin{array}{cc} 0 & \sigma^0 \\ \sigma^0 & 0 \end{array}\right), & 
  \gamma^{M\,j}=&\ \left(\begin{array}{cc} 0 & \sigma^j \\ -\sigma^j & 0 \end{array}\right), 
  \label{eq: Minkowski Dirac matrices} \\
  \gamma^{E\,0}=&\ \left(\begin{array}{cc} 0 & \sigma^0 \\ \sigma^0 & 0 \end{array}\right) = \gamma^{M\,0}, & 
  \gamma^{E\,j}=&\ \left(\begin{array}{cc} 0 & -i\sigma^j \\ i\sigma^j & 0 \end{array}\right) = -i\gamma^{M\,j},
  \label{eq: Euclidean Dirac matrices}
\end{align}\normalsize
which corresponds to the chiral representation in both Minkowski and Euclidean space-time. The Dirac matrix $ \gamma^0 $ is real, wheres the spatial Dirac matrices anti-hermitian in Minkowski space-time and hermitian in Euclidean space-time. They satisfy the Clifford algebra,
% \small
\begin{equation}
  \left\{\gamma^M_\mu,\gamma^M_\nu\right\} = 2g_{\mu\nu}, \quad
  \left\{\gamma^E_\mu,\gamma^E_\nu\right\} = 2\delta_{\mu\nu}.
\end{equation}\normalsize
The chirality matrix $ \gamma_5 $, which anticommutes with all Dirac matrices $ \gamma_\mu $, is defined by
% \small
\begin{equation}
  \gamma^M_5= i\gamma^{M\,0}\gamma^{M\,1}\gamma^{M\,2}\gamma^{M\,3}, \quad
  \gamma^E_5= \gamma^{E\,0}\gamma^{E\,1}\gamma^{E\,2}\gamma^{E\,3}
\end{equation}\normalsize
and is equal in Minkowski and Euclidean space-time:
\begin{equation}
  \gamma_5=\gamma^M_5=\gamma^E_5=\left(\begin{array}{cc} \sigma^0 & 0 \\ 0 & -\sigma^0 \end{array}\right).
\end{equation}
The chirality projectors are defined as
% \small
\begin{equation}
  P_R=\frac{1}{2}(1+\gamma_5),\quad P_L=\frac{1}{2}(1-\gamma_5)
  \label{eq: chirality projectors}
\end{equation}\normalsize
and parity projectors (for fermions) are defined as
% \small
\begin{equation}
  P_+=\frac{1}{2}(1+\gamma_0),\quad P_-=\frac{1}{2}(1-\gamma_0).
\end{equation}\normalsize
The charge conjugation matrix $ C $ is defined as
% \small
\begin{equation}
  C=i\gamma_0\gamma_2 = C^\dagger = C^{-1} =- C^T
  \label{eq: charge conjugation matrix}
\end{equation}\normalsize
both on Minkowski and Euclidean space-time and satisifies
% \small
\begin{equation}
  \gamma_\mu C = C^T\gamma_\mu^T.
\end{equation}\normalsize

\subsection{Continuous space-time and discrete space-time lattices}\label{app: Continuous space-time and discrete space-time lattices}
Events in a $ 4 $-dimensional continuous space-time $ V $ of infinite extent,
% \small
\begin{equation}
  V=\{x=(x_0,x_1,x_2,x_3)\ |\  -\infty<x_\mu<\infty\},
\end{equation}\normalsize
are labelled by $ 4 $-component coordinate vectors $ x $, which have the dimension of $ [\mathrm{length}] $. This definition can be restricted to any subspace of finite extent,
% \small
\begin{equation}
  V=\{x=(x_0,x_1,x_2,x_3)\ |\  0<x_\mu<L_\mu\},
\end{equation}\normalsize
where the size of the subspace introduces a length scale. Any finite subspace must be supplied with appropriate boundary conditions. Throughout this thesis, boundary conditions will be generally chosen as periodic or anti-periodic, e.g. any function satisfies
\begin{equation}
  f(x_\mu+L_\mu)= \pm f(x_\mu).
\end{equation}
In a discretisation, continuous space-time is replaced by a finite space-time lattice $ \Lambda $,
% \small
\begin{equation}
  \Lambda = \{ n=(n_0,n_1,n_2,n_3)\ |\ 0\leq n_\mu < N_\mu\}.
  \label{eq: Euclidean space-time lattice}
\end{equation}\normalsize
Events on this lattice are labelled by a $ 4 $-component site vector $ n $, which is dimensionless. It is connected to a coordinate vector of dimension $ [\mathrm{length}] $ as 
% \small
\begin{equation}
  x_\mu= a n_\mu
  \label{eq: site vectors}
\end{equation}
by a lattice spacing $ a $, which defines an intrinsic length scale of the system. Sites $ n $ of a discretised space-time lattice can be sorted into even and odd sites, which are distinguished by whether the sum of components
% \small
\begin{equation}
  n_\Sigma=\sum\limits_{\mu=0}^{3}n_\mu
  \label{eq: even-odd site number}
\end{equation}
is an even or an odd number. The volume is defined as $ V=a^4\,|\Lambda| $, where $ |\Lambda| = \prod_\mu N_\mu $ takes the role of a dimensionless volume. Slices of the lattice are defined for any direction by
% \small
\begin{equation}
  \Lambda_m^{\underline{\mu}} = \{n\in \Lambda\ | n_{\underline{\mu}} = m = \mathrm{const} \}.
  \label{eq: slices}
\end{equation}\normalsize


\sectionc{Fourier transformations}{app: Fourier transformations}
\noindent
Fourier transformations connect space-time $ V $ to its Fourier space $ \widetilde{V} $. 

\subsubsection{Infinite space-time}\label{app: Infinite continuous volume}
The Fourier space $ \widetilde{V} $ of an infinite space-time $ V $ is also infinite. The Fourier transform $ \widetilde{f}(p) $ of a real function $ f(x) $  is defined by
% \small
\begin{align}
  \widetilde{f}(p)=&\int\limits_{V} f(x) e^{-i x\cdot p} d^4x, \\
  f(x)=&\int\limits_{\widetilde{V}} \widetilde{f}(p) e^{i x\cdot p} \frac{d^4p}{(2\pi)^4}.
\end{align}\normalsize
Hence, complex functions $ \phi(x) $ are transformed to $ \widetilde{\phi}(p) $ according to
% \small
\begin{align}
  \widetilde{\phi}(p)=&\int\limits_{V} \phi(x) e^{-i x\cdot p} d^4x, \\
  \phi(x)=&\int\limits_{\widetilde{V}} \widetilde{\phi}(p) e^{i x\cdot p} \frac{d^4p}{(2\pi)^4}, \\
  \widetilde{\phi^\dagger}(p)=&\int\limits_{V} \phi^\dagger(x) e^{i x\cdot p} d^4x, \\
  \phi^\dagger(x)=&\int\limits_{\widetilde{V}} \widetilde{\phi^\dagger}(p) e^{-i x\cdot p} \frac{d^4p}{(2\pi)^4}.
\end{align}\normalsize
The Fourier transforms of the fields $ \psi $, $ \bar\psi $ and $ A $ are not marked with a tilde ($\,\widetilde{}\,$) explicitly. Delta functions, which naturally arise in Fourier transformations of local products of fields, are generated as
% \small
\begin{align}
  \delta(p-q)\equiv& \delta(p_0-q_0)\delta(p_1-q_1)\delta(p_2-q_2)\delta(p_3-q_3) = \int\limits_{V} e^{-i x\cdot (p-q)} d^4x, \label{eq: momentum delta function}\\
  \delta(x-y)\equiv& \delta(x_0-y_0)\delta(x_1-y_1)\delta(x_2-y_2)\delta(x_3-y_3) = \int\limits_{\widetilde{V}} e^{i (x-y)\cdot p} \frac{d^4p}{(2\pi)^4}. \label{eq: coordinate delta function}
\end{align}\normalsize

\subsubsection{Finite space-time lattice}
The discretised Fourier space is the Brillouin zone, $ \widetilde{V}=(2\pi/a)^4=|\Lambda|\,\prod_\mu(2\pi/(aN_\mu)) $. The Fourier transform $ f(k) $ of a real function $ f_n $ on a finite space-time lattice is defined by
% \small
\begin{align}
  \widetilde{f}(k)=&\frac{1}{\sqrt{|\Lambda|}}\sum\limits_{n \in \Lambda} f_n e^{-ia n\cdot k},   \label{eq: discrete Fourier transform}\\
  f_n=&\frac{1}{\sqrt{|\Lambda|}}\sum\limits_{k \in \widetilde{\Lambda}} \widetilde{f}(k) e^{ia n\cdot k}.
  \label{eq: inverse discrete Fourier transform}
\end{align}\normalsize
The equivalents of the delta functions of eq.s (\ref{eq: momentum delta function}) and (\ref{eq: coordinate delta function}) are given by
% \small
\begin{align}
  \delta(k,l)\equiv \delta_{k_0 l_0}\delta_{k_1 l_1}\delta_{k_2 l_2}\delta_{k_3 l_3} &= \frac{1}{|\Lambda|}\sum\limits_{n \in \Lambda} e^{-ia n\cdot (k-l)}, \label{eq: lattice momentum delta function}\\
  \delta_{n,m}\equiv \delta_{n_0 m_0}\delta_{n_1 m_1}\delta_{n_2 m_2}\delta_{n_3 m_3} &= \frac{1}{|\Lambda|}\sum\limits_{k \in \widetilde{\Lambda}} e^{ia (n-m)\cdot k}. \label{eq: site delta function}
\end{align}\normalsize
Generalisation of the (inverse) discrete Fourier transform of real functions to complex functions is analogous to the treatment in the continuous case (\mbox{cf.} \ref{app: Infinite continuous volume}).

